AcTracer: Active Testing of Large Language Model via Multi-Stage Sampling

Performance evaluation plays a crucial role in the development life cycle of large language models (LLMs). It estimates the model's capability, elucidates behavior characteristics, and facilitates the identification of potential issues and limitations, thereby guiding further improvement. Given that LLMs' diverse task-handling abilities stem from large volumes of training data, a comprehensive evaluation also necessitates abundant, well-annotated, and representative test data to assess LLM performance across various downstream tasks. However, the demand for high-quality test data often entails substantial time, computational resources, and manual efforts, sometimes causing the evaluation to be inefficient or impractical. To address these challenges, researchers propose active testing, which estimates the overall performance by selecting a subset of test data. Nevertheless, the existing active testing methods tend to be inefficient, even inapplicable, given the unique new challenges of LLMs (e.g., diverse task types, increased model complexity, and unavailability of training data). To mitigate such limitations and expedite the development cycle of LLMs, in this work, we introduce AcTracer, an active testing framework tailored for LLMs that strategically selects a small subset of test data to achieve a more accurate performance estimation for LLMs. AcTracer utilizes both internal and external information from LLMs to guide the test sampling process, reducing variance through a multi-stage pool-based active selection. Our experiment results demonstrate that AcTracer achieves state-of-the-art performance compared to existing methods across various tasks.

==> table/llm_performance.tex <==
\begin{table*}[h] %htbp
    \centering
    \renewcommand{\arraystretch}{0.8}
    %\scriptsize
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{cccccccccc}
    \toprule
         Dataset & AGIEval & TrivialQA & NQ-OPEN & GSM8K & TruthfulQA-I & TruthfulQA-T & HumanEval & MBPP  \\ \midrule
         
        %Metric & accuracy & exact match & exact match & exact match & info prob & truth prob & pass@1 & pass@1 \\ \midrule
        
        Mean & 0.2313 & 0.6414 & 0.1889 & 0.1440 & 0.8066 & 0.3390 & 0.3598 & 0.4060 \\ 
        
        Standard deviation & 0.4217 & 0.4796 & 0.3914 & 0.3511 & 0.1523 & 0.3076 & 0.4799 & 0.4911\\ \bottomrule
    \end{tabular}
    }
    \caption{Llama-2 and Code-Llama performance on all evaluated datasets \label{tab:llm_perf_llama2}}
\end{table*}



\begin{table*}[h] %htbp
    \centering
    \renewcommand{\arraystretch}{0.8}
    %\scriptsize
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{cccccccccc}
    \toprule
         Dataset & AGIEval & TrivialQA & NQ-OPEN & GSM8K & TruthfulQA-I & TruthfulQA-T & HumanEval & MBPP  \\ \midrule
         
        %Metric & accuracy & exact match & exact match & exact match & info prob & truth prob & pass@1 & pass@1 \\ \midrule
        
        Mean & 0.3022 & 0.7158 & 0.1343 & 0.4792 & 0.7901 & 0.3817 & 0.2561 & 0.3140 \\ 
        
        Standard deviation & 0.4592 & 0.4510 & 0.3410 & 0.4996 & 0.1699 & 0.3263 & 0.4365 & 0.4641\\ \bottomrule
    \end{tabular}
    }
    \caption{Llama-3 performance on all evaluated datasets \label{tab:llm_perf_llama3}}
\end{table*}
